An Age of Information Characterization of Frameless ALOHA

We provide a characterization of the peak age of information (AoI) achievable in a random-access system operating according to the frameless ALOHA protocol. Differently from previous studies, our analysis accounts for the fact that the number of terminals contending the channel may vary over time, as a function of the duration of the previous contention period. The exact characterization of the AoI provided in this paper, which is based on a Markovian analysis, reveals the impact of some key protocol parameters such as the maximum length of the contention period, on the average peak AoI. Specifically, we show that setting this parameter so as to maximize the throughput may result in an AoI degradation.

==> notation_v2.tex <==
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}

% Probability operators
\newcommand{\pr}{\ensuremath{\mathbb P}}
\newcommand{\expOp}{\ensuremath{\mathbb E}}

% Throughput, load
\newcommand{\tru}{\ensuremath{\mathsf S}}
\newcommand{\truSA}{\ensuremath{\mathsf S_{\mathsf{sa}}}}
\newcommand{\psSA}{\ensuremath{\mathsf p_{s,\mathsf{sa}}}}
\newcommand{\load}{\ensuremath{\mathsf G}}

% nodes in the network
\newcommand{\nodes}{\ensuremath{\mathsf U}}

% Markov process tracking active nodes
\newcommand{\nodesRV}{\ensuremath{N}}
\newcommand{\nodesRVl}{\ensuremath{\nodesRV^{(\ell)}}}
\newcommand{\nodesRVll}{\ensuremath{\nodesRV^{(\ell+1)}}}
\newcommand{\nodesrv}{\ensuremath{n}}

% Markov process tracking CP duration
\newcommand{\maxFrame}{\ensuremath{d_{\text{max}}}}
\newcommand{\cpRV}{\ensuremath{D}}
\newcommand{\cpRVl}{\ensuremath{\cpRV^{(\ell)}}}
\newcommand{\cpRVll}{\ensuremath{\cpRV^{(\ell+1)}}}
\newcommand{\cprv}{\ensuremath{d}}

% Markov process tracking number of decoded users per CP
\newcommand{\decRV}{\ensuremath{M}}
\newcommand{\decRVl}{\ensuremath{\decRV^{(\ell)}}}
\newcommand{\decrv}{\ensuremath{m}}

% Conditional probability of CP duration given contenders
\newcommand{\pDGivenN}{\ensuremath{P_{\cpRV|\nodesRV}}}
% Conditional probability of decoded users given contenders
\newcommand{\pMGivenN}{\ensuremath{P_{\decRV|\nodesRV}}}

\newcommand{\lsRV}{\ensuremath{Z}}
\newcommand{\lsRVn}{\ensuremath{\lsRV_n}}
\newcommand{\succRV}{\ensuremath{S}}
\newcommand{\succrv}{\ensuremath{s}}
\newcommand{\succRVn}{\ensuremath{\succRV_n}}

\newcommand{\pUGivenL}{\ensuremath{\mathsf p_{\nodesRV|\cpRV}}}
\newcommand{\pLGivenU}{\ensuremath{\mathsf p_{\cpRV|\nodesRV}}}
\newcommand{\pDecUsersGivenU}{\ensuremath{\mathsf p_s}}

\newcommand{\pActGivenL}{\ensuremath{\mathsf \gamma_{\cprv}}}
\newcommand{\pActGen}{\ensuremath{\mathsf \gamma}}

\newcommand{\driftU}{\ensuremath{\mathsf D_\nodesrv}}

\newcommand{\pAgeRV}{\ensuremath{A}}
\newcommand{\pAgerv}{\ensuremath{a}}
\newcommand{\inAgeRV}{\ensuremath{\pAgeRV_0}}
\newcommand{\inAgerv}{\ensuremath{\pAgerv_0}}
\newcommand{\fAgeRV}{\ensuremath{\pAgeRV_f}}
\newcommand{\sAgeRV}{\ensuremath{\pAgeRV_s}}
\newcommand{\sAgerv}{\ensuremath{\pAgerv_s}}
\newcommand{\fAgerv}{\ensuremath{\pAgerv_f}}

\newcommand{\firstCPRV}{\ensuremath{X}}
\newcommand{\firstCPrv}{\ensuremath{x}}
\newcommand{\firstCPSucc}{\ensuremath{\mathcal S_\firstCPrv}}
\newcommand{\firstCPFail}{\ensuremath{\mathcal F_\firstCPrv}}

\newcommand{\slots}{\ensuremath{\mathsf m}}
\newcommand{\pAct}{\ensuremath{\gamma}}
\newcommand{\pTx}{\ensuremath{q}}
\newcommand{\pUpdate}{\ensuremath{\nu}}
\newcommand{\psucc}{\ensuremath{\mathsf p_{\mathsf s}}}
\newcommand{\pdec}{\ensuremath{\mathsf p_{\mathsf d}}}
\newcommand{\pup}{\ensuremath{\mathsf p_{\mathsf{up}}}}

\newcommand{\tStamp}{\ensuremath{Y^{(i)}}}
\newcommand{\tGen}{\ensuremath{X^{(i)}}}

\newcommand{\age}{\ensuremath{\delta}}
\newcommand{\agei}{\ensuremath{\age^{(i)}}}
\newcommand{\Agei}{\ensuremath{\Delta^{(i)}}}
\newcommand{\AoI}{\ensuremath{\Delta}}

\newcommand{\actNodesFrame}{\ensuremath{N_a}}
\newcommand{\replicas}{\ensuremath{\ell}}
\newcommand{\tSlot}{\ensuremath{T_{\mathsf s}}}

% Markov chains
\newcommand{\pmc}[3]{\ensuremath{p_{#1}(#2,#3)}}

%finite length analysis
\newcommand{\unres}{\ensuremath{s}}
\newcommand{\collisions}{\ensuremath{c}}
\newcommand{\singletons}{\ensuremath{r}}
\newcommand{\au}{\ensuremath{i}}
\newcommand{\bu}{\ensuremath{j}}
\newcommand{\qu}{\ensuremath{h_\unres}}
\newcommand{\state}{\ensuremath{\Psi}}
\newcommand{\staten}[1]{\ensuremath{\state_{#1}}}
\newcommand{\stateafter}{\ensuremath{\Phi}}
\newcommand{\stateaftern}[1]{\ensuremath{\stateafter_{#1}}}

\newcommand{\prob}{\ensuremath{\mathbb P}}

%%%%%%%%%% AM
\newcommand{\peakAoI}{\ensuremath{\Omega}}
\newcommand{\avPeakAoI}{\ensuremath{{\peakAoI^*}}}
\newcommand{\initAoI}{\ensuremath{\AoI_0}}
\newcommand{\initaoi}{\ensuremath{\delta_0}}
\newcommand{\interUpdate}{\ensuremath{Y}}
\newcommand{\ancMC}{\ensuremath{Z}}
\newcommand{\ancmc}{\ensuremath{z}}
\newcommand{\ancMCl}{\ensuremath{\ancMC^{(\ell)}}
\newcommand{\ancMCll}{\ensuremath{\ancMC^{(\ell+1)}}
\newcommand{\succRVll}{\ensuremath{\succRV^{(\ell+1)}}


\newcommand{\decAtMaxFrame}{\ensuremath{\beta}}}
\newcommand{\ancRV}{\ensuremath{\zeta}}}


==> results.tex <==
\section{Results and Discussion}
\label{sec:results}

\am{Responsible: ANDREA/FRAN}
